Noisy-Pair Robust Representation Alignment for Positive-Unlabeled Learning

Positive-Unlabeled (PU) learning aims to train a binary classifier (positive vs. negative) where only limited positive data and abundant unlabeled data are available. While widely applicable, state-of-the-art PU learning methods substantially underperform their supervised counterparts on complex datasets, especially without auxiliary negatives or pre-estimated parameters (e.g., a 14.26% gap on CIFAR-100 dataset). We identify the primary bottleneck as the challenge of learning discriminative representations under unreliable supervision. To tackle this challenge, we propose NcPU, a non-contrastive PU learning framework that requires no auxiliary information. NcPU combines a noisy-pair robust supervised non-contrastive loss (NoiSNCL), which aligns intra-class representations despite unreliable supervision, with a phantom label disambiguation (PLD) scheme that supplies conservative negative supervision via regret-based label updates. Theoretically, NoiSNCL and PLD can iteratively benefit each other from the perspective of the Expectation-Maximization framework. Empirically, extensive experiments demonstrate that: (1) NoiSNCL enables simple PU methods to achieve competitive performance; and (2) NcPU achieves substantial improvements over state-of-the-art PU methods across diverse datasets, including challenging datasets on post-disaster building damage mapping, highlighting its promise for real-world applications. Code: Code will be open-sourced after review.

==> Tables/tab_L+Supervised.tex <==
\begin{table}[H]
\centering
\caption{Comparison of $\mathcal{L}_\text{r} $ and $\tilde{\mathcal{L}}_\text{r}$ in Supervised Learning.}
\label{tab_L+supervised}
\resizebox{\linewidth}{!}{%
\begin{tblr}{
  cells = {c},
  cell{1}{2} = {c=2}{},
  cell{1}{4} = {c=2}{},
  hline{1,3,5} = {-}{},
  hline{2} = {2-5}{},
}
                                              & CIFAR-10                    &                             & CIFAR-100                   &                             \\
                                              & OA                          & F1                          & OA                          & F1                          \\
$\mathcal{L}_\text{r}$             & 98.53\textsuperscript{±0.0} & 98.17\textsuperscript{±0.1} & 94.45\textsuperscript{±0.1} & 94.52\textsuperscript{±0.1} \\
$\tilde{\mathcal{L}}_\text{r}$ & 98.75\textsuperscript{±0.0} & 98.43\textsuperscript{±0.1} & 94.56\textsuperscript{±0.1} & 94.64\textsuperscript{±0.1} 
\end{tblr}
}
\end{table}

==> Tables/tab_L+other_method.tex <==
% \usepackage{tabularray}
\begin{table}
\centering
\caption{Performance of $\tilde{\mathcal{L}}_\text{r}$ with risk estimation (real $\pi_p$) and supervised methods.}
\label{tab_l_other_method}
\resizebox{\linewidth}{!}{%
\begin{tblr}{
  cells = {c},
  cell{1}{1} = {r=2}{},
  cell{1}{2} = {c=2}{},
  cell{1}{4} = {c=2}{},
  hline{1,3,7,9} = {-}{},
  hline{2} = {2-5}{},
}
Method                                    & CIFAR-10                    &                             & CIFAR-100                   &                             \\
                                          & OA                          & F1                          & OA                          & F1                          \\
uPU                                       & 69.43\textsuperscript{±0.3} & 41.32\textsuperscript{±1.0} & 61.68\textsuperscript{±0.9} & 44.18\textsuperscript{±2.6} \\
uPU+$\tilde{\mathcal{L}}_\text{r}$        & 97.35\textsuperscript{±0.1} & 96.66\textsuperscript{±0.2} & 83.71\textsuperscript{±1.6} & 81.40\textsuperscript{±2.2} \\
nnPU                                      & 83.25\textsuperscript{±0.2} & 76.94\textsuperscript{±0.5} & 71.22\textsuperscript{±0.5} & 68.12\textsuperscript{±1.0} \\
nnPU+$\tilde{\mathcal{L}}_\text{r}$       & 97.03\textsuperscript{±0.2} & 96.37\textsuperscript{±0.2} & 87.81\textsuperscript{±0.3} & 87.23\textsuperscript{±0.4} \\
Supervised+$\mathcal{L}_\text{r}$         & 98.53\textsuperscript{±0.0} & 98.17\textsuperscript{±0.1} & 94.45\textsuperscript{±0.1} & 94.52\textsuperscript{±0.1} \\
Supervised+$\tilde{\mathcal{L}}_\text{r}$ & 98.75\textsuperscript{±0.0} & 98.43\textsuperscript{±0.1} & 94.56\textsuperscript{±0.1} & 94.64\textsuperscript{±0.1} 
\end{tblr}
}
\end{table}

==> Tables/tab_L+risk.tex <==
\begin{table}[H]
\centering
\caption{Performance of $\tilde{\mathcal{L}}_\text{r}$ with risk estimation methods (real $\pi_p$).}
\label{tab_L+risk_estimation}
\resizebox{\linewidth}{!}{%
\begin{tabular}{ccccc} 
\hline
                                        & \multicolumn{2}{c}{CIFAR-10}                              & \multicolumn{2}{c}{CIFAR-100}                              \\ 
\cline{2-5}
                                        & OA                          & F1                          & OA                          & F1                           \\ 
\hline
uPU                                     & 69.43\textsuperscript{±0.3} & 41.32\textsuperscript{±1.0} & 61.68\textsuperscript{±0.9} & 44.18\textsuperscript{±2.6}  \\
uPU+$\tilde{\mathcal{L}}_\text{r}$  & 97.35\textsuperscript{±0.1} & 96.66\textsuperscript{±0.2} & 83.71\textsuperscript{±1.6} & 81.40\textsuperscript{±2.2}  \\ 
\hline
nnPU                                    & 83.25\textsuperscript{±0.2} & 76.94\textsuperscript{±0.5} & 71.22\textsuperscript{±0.5} & 68.12\textsuperscript{±1.0}  \\
nnPU+$\tilde{\mathcal{L}}_\text{r}$ & 97.03\textsuperscript{±0.2} & 96.37\textsuperscript{±0.2} & 87.81\textsuperscript{±0.3} & 87.23\textsuperscript{±0.4}  \\
\hline
\end{tabular}
}
\end{table}

==> Tables/tab_ablation.tex <==
% \usepackage{tabularray}
\begin{table}
\centering
\caption{Ablation and comparative analyses on the CIFAR-100 dataset.}
\label{tab_ablation_study}
\resizebox{0.5\linewidth}{!}{%
\begin{tblr}{
  cells = {c},
  hline{1-2,4,8-9} = {-}{},
}
NCL                            & LD             & OA                          & F1                           & P                           & R                            \\
                               & $s$            & 61.54\textsuperscript{±7.8} & 40.58\textsuperscript{±22.9} & 84.36\textsuperscript{±7.1} & 30.69\textsuperscript{±25.0} \\
$\tilde{\mathcal{L}}_\text{r}$ &                & 50.27\textsuperscript{±0.1} & 1.09\textsuperscript{±0.4}   & 97.97\textsuperscript{±1.8} & 0.55\textsuperscript{±0.2}   \\
$\mathcal{L}_\text{self-r}$    & $s$            & 73.22\textsuperscript{±1.7} & 72.75\textsuperscript{±1.6}  & 74.10\textsuperscript{±2.2} & 71.47\textsuperscript{±1.9}  \\
$\mathcal{L}_\text{r}$         & $s$            & 84.58\textsuperscript{±0.8} & 85.90\textsuperscript{±0.6}  & 79.12\textsuperscript{±1.1} & 93.96\textsuperscript{±0.3}  \\
$\tilde{\mathcal{L}}_\text{r}$ & $s^\prime$     & 75.14\textsuperscript{±2.7} & 79.91\textsuperscript{±1.7}  & 67.15\textsuperscript{±2.6} & 98.73\textsuperscript{±0.5}  \\
$\tilde{\mathcal{L}}_\text{r}$ & $s^\prime$+SAT & 50.25\textsuperscript{±0.0} & 1.01\textsuperscript{±0.1}   & 97.85\textsuperscript{±3.7} & 0.51\textsuperscript{±0.1}   \\
$\tilde{\mathcal{L}}_\text{r}$ & $s$            & 88.28\textsuperscript{±0.6} & 88.14\textsuperscript{±0.9}  & 89.12\textsuperscript{±1.7} & 87.27\textsuperscript{±3.2}  
\end{tblr}
}
\end{table}
